MTLDesc: Looking Wider to Describe Better

Limited by the locality of convolutional neural networks, most existing local features description methods only learn local descriptors with local information and lack awareness of global and surrounding spatial context. In this work, we focus on making local descriptors "look wider to describe better" by learning local Descriptors with More Than just Local information (MTLDesc). Specifically, we resort to context augmentation and spatial attention mechanisms to make our MTLDesc obtain non-local awareness. First, Adaptive Global Context Augmented Module and Diverse Local Context Augmented Module are proposed to construct robust local descriptors with context information from global to local. Second, Consistent Attention Weighted Triplet Loss is designed to integrate spatial attention awareness into both optimization and matching stages of local descriptors learning. Third, Local Features Detection with Feature Pyramid is given to obtain more stable and accurate keypoints localization. With the above innovations, the performance of our MTLDesc significantly surpasses the prior state-of-the-art local descriptors on HPatches, Aachen Day-Night localization and InLoc indoor localization benchmarks.

==> table_data.tex <==
\begin{table}[h]
\resizebox{\linewidth}{!}{
\begin{tabular}{|c|c|c|c|}
\hline
Method     & Source                                                          & Images          & MMA@3          \\ \hline
SuperPoint & COCO                                                            & 80,000          & 0.645          \\ \hline
D2Net      & MegaDepth                                                       & 617,774         & 0.429          \\ \hline
R2D2       & \begin{tabular}[c]{@{}c@{}}Aachen and\\ Web images\end{tabular} & \textbf{12,083} & 0.686          \\ \hline
ASLFeat    & GL3D                                                            & 1600,000        & 0.723          \\ \hline
MTLDesc    & MegaDepth                                                       & 23,600          & \textbf{0.787} \\ \hline
\end{tabular}
}
\caption{Comparisons on the Training Dataset Settings. 
Source refers to the training data.
\textit{MMA}@3 is the mean matching accuracy evaluated on the HPatches datasets~\cite{hpatches} with single scale input.
}
\label{tab:abl}
\end{table}


==> table_inloc.tex <==
\begin{table}[thb]
\centering
\resizebox{\linewidth}{!}{
\begin{tabular}{ccccccc}
\hline
\multicolumn{7}{c}{\textbf{InLoc benchmark}} \\ \hline
\multicolumn{1}{c|}{\multirow{2}{*}{\textbf{{Method}}}} & \multicolumn{6}{c}{\textbf{{Localized queries}}\emph{(\%, 0.25m/0.5m/1.0m)}} \\ \cline{2-7} 
\multicolumn{1}{c|}{} & \multicolumn{3}{c|}{\textbf{{DUC1}}} & \multicolumn{3}{c}{\textbf{{DUC2}}} \\ \hline
\multicolumn{1}{c|}{SuperPoint} & 39.9 & 55.6 & \multicolumn{1}{c|}{67.2} & 37.4 & 57.3 & \textbf{70.2} \\
\multicolumn{1}{c|}{D2Net} & 39.9 & 57.6 & \multicolumn{1}{c|}{67.2} & 36.6 & 53.4 & 61.8 \\
\multicolumn{1}{c|}{R2D2} & 36.4 & 57.1 & \multicolumn{1}{c|}{\textbf{73.7}} & 44.3 & 60.3 & 68.7 \\
\multicolumn{1}{c|}{ASLFeat} & 36.4 & 56.1 & \multicolumn{1}{c|}{66.7} & 36.6 & 55.7 & 61.1 \\ 
\multicolumn{1}{c|}{CAPS + SuperPoint} & 32.8 & 53.0 & \multicolumn{1}{c|}{64.6} & 32.8 & {58.8} & 64.1 \\
\multicolumn{1}{c|}{DISK} & 38.9 & 59.1 & \multicolumn{1}{c|}{67.7} & 37.4 & 57.3 & 64.1 \\
\hline
\multicolumn{1}{c|}{MTLFeat} & \textbf{41.9} & \textbf{61.6} & \multicolumn{1}{c|}{72.2} & \textbf{45.0} & \textbf{61.1} & \textbf{70.2} \\ \hline
\end{tabular}

}
\begin{tabular}{c}
    \\
\end{tabular}

\caption{
Evaluation results of the InLoc dataset.
We report the percentage of correctly localized queries under specific error thresholds for each method. 
%Ablation on the Sampling Strategy.
%The model with the Keypoints Guided Sampling leads to better performance, demonstrating that the descriptors training with the proposed strategy are more consistent with the detected keypoints.
}
\label{tab:inloc}
\end{table}




==> table_time.tex <==
\begin{table}[h]
\resizebox{\linewidth}{!}{
\begin{tabular}{|c|c|l|l|l|l|}
\hline
Method & SuperPoint & D2Net & R2D2  & ASLFeat & MTLDesc \\ \hline
Speed  & {\bf 31 FPS}     & 6 FPS & 8 FPS & 21 FPS  &  24 FPS  \\ \hline
\end{tabular}
}

\caption{Comparisons on the Running Speed. The speed is averaged on HPatches (480 × 640) with same setting.
}
\label{table:time}
\end{table}

